When Does Visual Prompting Outperform Linear Probing for Vision-Language Models? A Likelihood Perspective

Adapting pre-trained models to new tasks can exhibit varying effectiveness across datasets. Visual prompting, a state-of-the-art parameter-efficient transfer learning method, can significantly improve the performance of out-of-distribution tasks. On the other hand, linear probing, a standard transfer learning method, can sometimes become the best approach. We propose a log-likelihood ratio (LLR) approach to analyze the comparative benefits of visual prompting and linear probing. By employing the LLR score alongside resource-efficient visual prompts approximations, our cost-effective measure attains up to a 100-fold reduction in run time compared to full training, while achieving prediction accuracies up to 91%. The source code is available at https://github.com/IBM/VP-LLR.

==> tables/accuracy.tex <==
\begin{table*}[t]
\caption{The LLR-Accuracy. The highest score is marked in \textbf{bold} (excluding scores from trained prompts).}
\label{tab:acc}
\centering
\renewcommand{\arraystretch}{1.25}
\begin{tabular}{c|cccccc}
\hline
 & \begin{tabular}[c]{@{}c@{}}Trained\\ Prompts\end{tabular} & \begin{tabular}[c]{@{}c@{}}Without\\ Prompts\end{tabular} & Guassian & Gradient & Mini-Finetune & \begin{tabular}[c]{@{}c@{}}Mini-Finetune\\ 5 Rounds\end{tabular} \\ \hline
ResNet18 & 75.0 & 41.7 & \textbf{58.3} & \textbf{58.3} & \textbf{58.3} & \textbf{58.3} \\ \hline
ResNext-IG & 83.3 & 50.0 & 66.7 & \textbf{83.3} & 58.3 & 58.3 \\ \hline
ViT-B-16 & 66.7 & 75.0 & \textbf{91.7} & \textbf{91.7} & \textbf{91.7} & \textbf{91.7} \\ \hline
Swin-T & 91.7 & 50.0 & 83.3 & 83.3 & 83.3 & \textbf{91.7} \\ \hline
CLIP(VIT/B-32) & 83.3 & 50.0 & 66.7 & 66.7 & 66.7 & \textbf{75.0} \\ \hline
\end{tabular}
\end{table*}

==> tables/kendall.tex <==
\begin{table*}[t]
\caption{The Kendall's $\tau$ coefficient. The highest score is marked in \textbf{bold} (excluding scores from trained prompts). We utilize several OOD detection methods as our baselines, including the confidence score \cite{hendrycks2016baseline}, entropy, and the confidence score obtained from ODIN \cite{liang2017enhancing}.} \label{tab:kendall}
\centering
\renewcommand{\arraystretch}{1.25}
\resizebox{.9\textwidth}{!}{
\begin{tabular}{c|cccccc|cccc}
\hline
 & \begin{tabular}[c]{@{}c@{}}Trained\\ Prompts\end{tabular} & \begin{tabular}[c]{@{}c@{}}Without\\ Prompts\end{tabular} & Gaussian & Gradient & Mini-Finetune & \begin{tabular}[c]{@{}c@{}}Mini-Finetune\\ 5 Rounds\end{tabular} & \begin{tabular}[c]{@{}c@{}}Confidence \\ Score\end{tabular} & Entropy & \begin{tabular}[c]{@{}c@{}}ODIN \\ Confidence \end{tabular}& \begin{tabular}[c]{@{}c@{}}Mahalanobis Distance \\ AUROC\end{tabular}\\ \hline
ResNet18 & 0.61 & \textbf{0.67} & 0.48 & 0.52 & 0.42 & 0.45 & 0.27 & 0.21 & 0.21 & 0.52\\ \hline
ResNext-IG & 0.58 & 0.18 & 0.61 & \textbf{0.64} & 0.33 & 0.27 & 0.52 & 0.52 & 0.33 & 0.38\\ \hline
ViT-B-16 & 0.61 & 0.42 & 0.58 & \textbf{0.64} & 0.48 & 0.48 & 0.18 & -0.09 &-0.18 & 0.61\\ \hline
Swin-T & 0.58 & 0.39 & 0.42 & 0.42 & 0.48 & \textbf{0.70} & 0.48 &  0.52 & 0.39 & 0.52\\ \hline
CLIP(VIT/B-32) & 0.64 & 0.27 & 0.55 & 0.55 & \textbf{0.61} & 0.52 & 0.39 &  0.30 & 0.15 & 0.45\\ \hline
\end{tabular}
}
\end{table*}

==> tables/spearman.tex <==
\vspace{-2mm}
\begin{table*}[t]
\caption{The Spearman's $\rho$ coefficient. The highest score is marked in \textbf{bold} (excluding scores from trained prompts).}  \label{tab:spearman}
\vspace{2mm}
\centering
\renewcommand{\arraystretch}{1.25}
\resizebox{.9\textwidth}{!}{
\begin{tabular}{c|cccccc|cccc}
\hline
 & \begin{tabular}[c]{@{}c@{}}Trained\\ Prompts\end{tabular} & \begin{tabular}[c]{@{}c@{}}Without\\ Prompts\end{tabular} & Gaussian & Gradient & Mini-Finetune & \begin{tabular}[c]{@{}c@{}}Mini-Finetune\\ 5 Rounds\end{tabular} & \begin{tabular}[c]{@{}c@{}}Confidence\\ Score\end{tabular} & Entropy & \begin{tabular}[c]{@{}c@{}}ODIN \\ Confidence\end{tabular} & \begin{tabular}[c]{@{}c@{}}Mahalanobis Distance \\ AUROC\end{tabular}\\ \hline
ResNet18 & 0.77 & \textbf{0.83} & 0.65 & 0.71 & 0.62 & 0.61 & 0.41 & 0.38 & 0.31 & 0.69\\ \hline
ResNext-IG & 0.78 & 0.24 & 0.73 & \textbf{0.80} & 0.48 & 0.38 & 0.70 & 0.70 & 0.47 & 0.60\\ \hline
ViT-B-16 & 0.81 & 0.66 & 0.77 & \textbf{0.82} & 0.63 & 0.64 & 0.18 & -0.16 & -0.31 & 0.77\\ \hline
Swin-T & 0.80 & 0.56 & 0.67 & 0.63 & 0.69 & \textbf{0.81} & 0.73 &  0.75 & 0.59 & 0.73\\ \hline
CLIP(VIT/B-32) & 0.84 & 0.38 & 0.73 & 0.69 & \textbf{0.79} & 0.71 & 0.62 & 0.48 & 0.15 & 0.61\\ \hline
\end{tabular}
}
\end{table*}
